The Moral Turing Test: Evaluating Human-LLM Alignment in Moral Decision-Making

As large language models (LLMs) become increasingly integrated into society, their alignment with human morals is crucial. To better understand this alignment, we created a large corpus of human- and LLM-generated responses to various moral scenarios. We found a misalignment between human and LLM moral assessments; although both LLMs and humans tended to reject morally complex utilitarian dilemmas, LLMs were more sensitive to personal framing. We then conducted a quantitative user study involving 230 participants (N=230), who evaluated these responses by determining whether they were AI-generated and assessed their agreement with the responses. Human evaluators preferred LLMs' assessments in moral scenarios, though a systematic anti-AI bias was observed: participants were less likely to agree with judgments they believed to be machine-generated. Statistical and NLP-based analyses revealed subtle linguistic differences in responses, influencing detection and agreement. Overall, our findings highlight the complexities of human-AI perception in morally charged decision-making.

==> tables_bg.tex <==
\begin{tabular}{lllllllll}
\toprule
 & Exp. & A & B & T & dof & p-corr & cohen & BF_{10} \\
\midrule
1 & $\text{all}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-14.64$ & $152.0$ & $p < 0.001$ & $-1.67$ & $4.092\times 10^{27}$ \\
2 & $\text{all}$ & $\text{chance}$ & $\text{non moral}$ & $-14.15$ & $152.0$ & $p < 0.001$ & $-1.62$ & $2.165\times 10^{26}$ \\
3 & $\text{all}$ & $\text{chance}$ & $\text{personal moral}$ & $-12.46$ & $152.0$ & $p < 0.001$ & $-1.42$ & $7.261\times 10^{21}$ \\
4 & $\text{all}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $3.51$ & $152.0$ & $p < 0.01$ & $0.33$ & $30.066}$ \\
5 & $\text{all}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $0.22$ & $152.0$ & $p = 1.00$ & $0.02$ & $0.092}$ \\
6 & $\text{all}$ & $\text{non moral}$ & $\text{personal moral}$ & $-3.07$ & $152.0$ & $p < 0.05$ & $-0.28$ & $8.0}$ \\
7 & $\text{dv2}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-8.9$ & $76.0$ & $p < 0.001$ & $-1.43$ & $3.687\times 10^{10}$ \\
8 & $\text{dv2}$ & $\text{chance}$ & $\text{non moral}$ & $-9.56$ & $76.0$ & $p < 0.001$ & $-1.54$ & $6.198\times 10^{11}$ \\
9 & $\text{dv2}$ & $\text{chance}$ & $\text{personal moral}$ & $-7.24$ & $76.0$ & $p < 0.001$ & $-1.17$ & $3.204\times 10^{07}$ \\
10 & $\text{dv2}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $0.82$ & $76.0$ & $p = 1.00$ & $0.1$ & $0.173}$ \\
11 & $\text{dv2}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $0.71$ & $76.0$ & $p = 1.00$ & $0.09$ & $0.16}$ \\
12 & $\text{dv2}$ & $\text{non moral}$ & $\text{personal moral}$ & $0.04$ & $76.0$ & $p = 1.00$ & $0.0$ & $0.126}$ \\
13 & $\text{dv3}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-12.22$ & $75.0$ & $p < 0.001$ & $-1.98$ & $3.19\times 10^{16}$ \\
14 & $\text{dv3}$ & $\text{chance}$ & $\text{non moral}$ & $-10.43$ & $75.0$ & $p < 0.001$ & $-1.69$ & $2.112\times 10^{13}$ \\
15 & $\text{dv3}$ & $\text{chance}$ & $\text{personal moral}$ & $-10.78$ & $75.0$ & $p < 0.001$ & $-1.75$ & $9.05\times 10^{13}$ \\
16 & $\text{dv3}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $3.94$ & $75.0$ & $p < 0.01$ & $0.57$ & $116.473}$ \\
17 & $\text{dv3}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $-0.42$ & $75.0$ & $p = 1.00$ & $-0.05$ & $0.137}$ \\
18 & $\text{dv3}$ & $\text{non moral}$ & $\text{personal moral}$ & $-4.53$ & $75.0$ & $p < 0.001$ & $-0.56$ & $819.582}$ \\
\bottomrule
\caption{P(correct)}
\end{tabular}


\begin{tabular}{lllllllll}
\toprule
 & Exp. & A & B & T & dof & p-corr & cohen & BF_{10} \\
\midrule
1 & $\text{all}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-1.74$ & $152.0$ & $p = 0.51$ & $-0.2$ & $0.39}$ \\
2 & $\text{all}$ & $\text{chance}$ & $\text{non moral}$ & $-5.13$ & $152.0$ & $p < 0.001$ & $-0.59$ & $1.355\times 10^{04}$ \\
3 & $\text{all}$ & $\text{chance}$ & $\text{personal moral}$ & $4.35$ & $152.0$ & $p < 0.001$ & $0.5$ & $586.852}$ \\
4 & $\text{all}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $-1.93$ & $152.0$ & $p = 0.33$ & $-0.21$ & $0.55}$ \\
5 & $\text{all}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $4.69$ & $152.0$ & $p < 0.001$ & $0.49$ & $2180.903}$ \\
6 & $\text{all}$ & $\text{non moral}$ & $\text{personal moral}$ & $6.87$ & $152.0$ & $p < 0.001$ & $0.76$ & $5.329\times 10^{07}$ \\
7 & $\text{dv2}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-0.07$ & $76.0$ & $p = 1.00$ & $-0.01$ & $0.126}$ \\
8 & $\text{dv2}$ & $\text{chance}$ & $\text{non moral}$ & $-4.64$ & $76.0$ & $p < 0.001$ & $-0.75$ & $1235.799}$ \\
9 & $\text{dv2}$ & $\text{chance}$ & $\text{personal moral}$ & $1.92$ & $76.0$ & $p = 0.70$ & $0.31$ & $0.721}$ \\
10 & $\text{dv2}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $-2.66$ & $76.0$ & $p = 0.12$ & $-0.41$ & $3.281}$ \\
11 & $\text{dv2}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $1.35$ & $76.0$ & $p = 1.00$ & $0.21$ & $0.3}$ \\
12 & $\text{dv2}$ & $\text{non moral}$ & $\text{personal moral}$ & $4.19$ & $76.0$ & $p < 0.001$ & $0.71$ & $263.91}$ \\
13 & $\text{dv3}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-2.56$ & $75.0$ & $p = 0.15$ & $-0.42$ & $2.654}$ \\
14 & $\text{dv3}$ & $\text{chance}$ & $\text{non moral}$ & $-2.81$ & $75.0$ & $p = 0.08$ & $-0.46$ & $4.73}$ \\
15 & $\text{dv3}$ & $\text{chance}$ & $\text{personal moral}$ & $4.15$ & $75.0$ & $p < 0.01$ & $0.67$ & $232.239}$ \\
16 & $\text{dv3}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $-0.07$ & $75.0$ & $p = 1.00$ & $-0.01$ & $0.127}$ \\
17 & $\text{dv3}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $5.77$ & $75.0$ & $p < 0.001$ & $0.78$ & $7.976\times 10^{04}$ \\
18 & $\text{dv3}$ & $\text{non moral}$ & $\text{personal moral}$ & $5.52$ & $75.0$ & $p < 0.001$ & $0.81$ & $3.063\times 10^{04}$ \\
\bottomrule
\caption{Bias (source)}
\end{tabular}


\begin{tabular}{lllllllll}
\toprule
 & Exp. & A & B & T & dof & p-corr & cohen & $BF_{10}$ \\
\midrule
1 & $\text{all}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-2.71$ & $143.0$ & $p < 0.05$ & $-0.32$ & $3.087}$ \\
2 & $\text{all}$ & $\text{chance}$ & $\text{non moral}$ & $-5.76$ & $143.0$ & $p < 0.001$ & $-0.68$ & $2.198\times 10^{05}$ \\
3 & $\text{all}$ & $\text{chance}$ & $\text{personal moral}$ & $-4.31$ & $143.0$ & $p < 0.001$ & $-0.51$ & $498.6}$ \\
4 & $\text{all}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $-2.13$ & $143.0$ & $p = 0.21$ & $-0.23$ & $0.83}$ \\
5 & $\text{all}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $-1.18$ & $143.0$ & $p = 1.00$ & $-0.11$ & $0.184}$ \\
6 & $\text{all}$ & $\text{non moral}$ & $\text{personal moral}$ & $1.19$ & $143.0$ & $p = 1.00$ & $0.12$ & $0.184}$ \\
7 & $\text{dv2}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-2.08$ & $73.0$ & $p = 0.49$ & $-0.34$ & $0.973}$ \\
8 & $\text{dv2}$ & $\text{chance}$ & $\text{non moral}$ & $-3.86$ & $73.0$ & $p < 0.01$ & $-0.63$ & $90.741}$ \\
9 & $\text{dv2}$ & $\text{chance}$ & $\text{personal moral}$ & $-5.16$ & $73.0$ & $p < 0.001$ & $-0.85$ & $7759.918}$ \\
10 & $\text{dv2}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $-1.4$ & $73.0$ & $p = 1.00$ & $-0.21$ & $0.324}$ \\
11 & $\text{dv2}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $-2.61$ & $73.0$ & $p = 0.13$ & $-0.34$ & $2.948}$ \\
12 & $\text{dv2}$ & $\text{non moral}$ & $\text{personal moral}$ & $-0.84$ & $73.0$ & $p = 1.00$ & $-0.12$ & $0.18}$ \\
13 & $\text{dv3}$ & $\text{chance}$ & $\text{impersonal moral}$ & $-1.72$ & $69.0$ & $p = 1.00$ & $-0.29$ & $0.532}$ \\
14 & $\text{dv3}$ & $\text{chance}$ & $\text{non moral}$ & $-4.42$ & $69.0$ & $p < 0.001$ & $-0.75$ & $534.395}$ \\
15 & $\text{dv3}$ & $\text{chance}$ & $\text{personal moral}$ & $-0.66$ & $69.0$ & $p = 1.00$ & $-0.11$ & $0.162}$ \\
16 & $\text{dv3}$ & $\text{impersonal moral}$ & $\text{non moral}$ & $-1.63$ & $69.0$ & $p = 1.00$ & $-0.26$ & $0.462}$ \\
17 & $\text{dv3}$ & $\text{impersonal moral}$ & $\text{personal moral}$ & $1.06$ & $69.0$ & $p = 1.00$ & $0.15$ & $0.224}$ \\
18 & $\text{dv3}$ & $\text{non moral}$ & $\text{personal moral}$ & $2.95$ & $69.0$ & $p = 0.05$ & $0.46$ & $6.824}$ \\
\bottomrule
\caption{Bias (belief)}
\end{tabular}

